Tensor-Aware Energy Accounting

With the rapid growth of Artificial Intelligence (AI) applications supported by deep learning (DL), the energy efficiency of these applications has an increasingly large impact on sustainability. We introduce Smaragdine, a new energy accounting system for tensor-based DL programs implemented with TensorFlow. At the heart of Smaragdine is a novel white-box methodology of energy accounting: Smaragdine is aware of the internal structure of the DL program, which we call tensor-aware energy accounting. With Smaragdine, the energy consumption of a DL program can be broken down into units aligned with its logical hierarchical decomposition structure. We apply Smaragdine for understanding the energy behavior of BERT, one of the most widely used language models. Layer-by-layer and tensor-by-tensor, Smaragdine is capable of identifying the highest energy/power-consuming components of BERT. Furthermore, we conduct two case studies on how Smaragdine supports downstream toolchain building, one on the comparative energy impact of hyperparameter tuning of BERT, the other on the energy behavior evolution when BERT evolves to its next generation, ALBERT.

==> src/notes.tex <==
\section{Notes for \ourframework{} + tensorflow}

\subsection{Comparison of Input Dataset}

This section presents experiments comparing different inputs with the same model.

\subsection{Comparison of Training vs Inference}

This section presents experiments comparing training and inference for the same input + model.

\subsection{Comparison of Models}

This section presents experiments comparing different models with the same input.

\subsection{Exploration of Hyperparameters}

This section presents experiments comparing models with different hyperparameters.

\subsection{What does the data need?}

The end goal of this project is to leverage \ourframework{}'s footprints to program against top methods. 

Based on the overview of data above, it sounds like we are doing dimensionality searches. For example, if we explore \textsc{BERT} (https://github.com/google-research/bert), we would want to run the experiments from their presented scores:

\begin{center}
    \begin{tabular}{ c | c | c | c | c | c | c | c | c | c | c | c | c }
      \textbf{Model} & \textbf{Score} & \textbf{CoLA} & \textbf{SST-2} & \textbf{MRPC} & \textbf{STS-B} & \textbf{QQP} & \textbf{MNLI-m} & \textbf{MNLI-mm} & \textbf{QNLI(v2)} & \textbf{RTE} & \textbf{WNLI} & \textbf{AX} \\
      \hline
      \textsc{BERT}-Tiny & 64.2 & 0.0 & 83.2 & 81.1/71.1 & 74.3/73.6 & 62.2/83.4 & 70.2 & 70.3 & 81.5 & 57.2 & 62.3 & 21.0 \\
      \textsc{BERT}-Mini & 65.8 & 0.0 & 85.9 & 81.1/71.8 & 75.4/73.3 & 66.4/86.2 & 74.8 & 74.3 & 84.1 & 57.9 & 62.3 & 26.1 \\
      \textsc{BERT}-Small & 71.2 & 27.8 & 89.7 & 83.4/76.2 & 78.8/77.0 & 68.1/87.0 & 77.6 & 77.0 & 86.4 & 61.8 & 62.3 & 28.6 \\
      \textsc{BERT}-Medium & 73.5 & 38.0 & 89.6 & 86.6/81.6 & 80.4/78.4 & 69.6/87.9 & 80.0 & 79.1 & 87.7 & 62.2 & 62.3 & 30.5
    \end{tabular}
\end{center}

This is a grid experiment that we would run around the entire training experiment/script depending on what we want to capture. Since we want to compare training and inference, eflect needs to be able to profile within the script instead of around the runtime. Maybe a future student can explore if the training and inference stages can be differentiated from each other from outside the runtime.

Given that the medium size runs for 20 minutes, this would mean we are collecting on the order of 4-5 hours of data just for one experiment. We should be smart about our experiments so that we don't have to re-collect often.

We are comparing logical behavior, so we are probably presenting similar data to \textsc{Chappie}: method/class/package rankings and context-sensitivities. We can compute the correlations to compare the experiments. As a result, we construct a correlation hyperspace. This is similar to the baseline comparisons we've done up to now but in this case there is no baseline. Since we are comparing profiled runtimes, we have to consider the entire hyperspace. From there, we would explore specific slices of the hyperspace. 

In the case of \textsc{BERT}, we have two primary dimensions: the hyperparameters and the dataset. This also bring up the question of how to compare inference. I think we can compare two inference runtimes with different settings and the inference runtime with its training runtime but nothing beyond that.

For \textsc{BERT}, I think we should present two types of comparison data. This can just be a correlation of the method ranking but we can compare anything we like here. The first one is a grid showing the method comparisons between any two hyperparameter settings. The second one is a list of comparisons between the training and inference runtimes. Therefore, we would have a measure of similarity between runtime settings.

For other experiments, we can do the same thing. If we use the image recognition models provided by \texttt{tensorflow-slim}, we can compute the same comparison metrics we did above.
